"If sighted people know, I should be able to know:" Privacy Perceptions of Bystanders with Visual Impairments around Camera-based Technology

Camera-based technology can be privacy-invasive, especially for bystanders who can be captured by the cameras but do not have direct control or access to the devices. The privacy threats become even more significant to bystanders with visual impairments (BVI) since they cannot visually discover the use of cameras nearby and effectively avoid being captured. While some prior research has studied visually impaired people's privacy concerns as direct users of camera-based assistive technologies, no research has explored their unique privacy perceptions and needs as bystanders. We conducted an in-depth interview study with 16 visually impaired participants to understand BVI's privacy concerns, expectations, and needs in different camera usage scenarios. A preliminary survey with 90 visually impaired respondents and 96 sighted controls was conducted to compare BVI and sighted bystanders' general attitudes towards cameras and elicit camera usage scenarios for the interview study. Our research revealed BVI's unique privacy challenges and perceptions around cameras, highlighting their needs for privacy awareness and protection. We summarized design considerations for future privacy-enhancing technologies to fulfill BVI's privacy needs.

==> 2-tables/codebook.tex <==

\begin{table*}
  \centering
  \setlength{\tabcolsep}{2.5pt}
  % \renewcommand{\arraystretch}{1.2}
  % \resizebox{\textwidth}{!}{%
      \small
    \begin{tabular}{m{10em}     % themes
                    m{15em}     % subthemes 
                    m{25em}}      % codes
    &&&
   % \multicolumn{4}{c}{\textbf{Deployability}} &
   % \multicolumn{7}{c}{\textbf{Usability}} &
   % \multicolumn{5}{c}{\textbf{Accessibility}} &
   % \multicolumn{4}{c}{\textbf{Security}} \\
   % \cmidrule{5-24}
    \textbf{Themes}& \textbf{Sub-themes} & \textbf{Codes}\\
    \midrule
    %
    %%%%%%%%%%%%%%%%%%%%%%%%%%
    % PHYSICAL BIOMETRICS
    %%%%%%%%%%%%%%%%%%%%%%%%%%
    %
    \multirow{13}{10em}{No Agency to Detect/Avoid Cameras} 
    &  
    No access to camera info  & unable to detect; camera presence; camera location; camera range; unable to avoid; no control; frustrating; lack of agency\\ 
    \cline{2-3}
    &
    Passively infer camera usage  & audio cues; shutter sound; audio cue not effective; audio muted; hard to hear; hard to distinguish source; overhear conversation; notified by others; do not expect cam user to inform; hard to form privacy opinion \\ 
    \cline{2-3}
    &
    Communication to protect privacy  & communicate with cam user; ask for info; negotiate for agreement; confront; withdraw oneself; resignation; avoidance; unable to communicate; unwilling to communicate; information uncertainty; confirm camera users' behaviors; no control \\ 
    \cline{2-3}
    &
    Unique challenges of low vision & visual cues; light indicator; smartglasses vs normal glasses; body language of using camera; small; invisible; wearable camera harder to see \\
    \midrule
    %
    \multirow{8}{10em}{Adapted Privacy Perceptions} 
    &  
    Common perception  & public camera; public place; uncomfortable with personal camera; intentional; uncomfortable with private place; disguised cam; malicious purpose; compromise to social norms; uncomfortable at first; get used to cam; \\ 
    \cline{2-3}
    &
    Low privacy expectation  & low privacy expectation; self-regulation; expect no privacy; assume camera everywhere; no concerns; self-blame; put sensitive info away;   \\ 
    \cline{2-3}
    &
    High trust on acquaintances  & trust acquaintances; assume harmless purpose; easy to communicate with acquaintances; more likely be informed; willing to accommodate; cautious about strangers; check photos \\ 
    \midrule
    %
    \multirow{8}{10em}{Empathy towards Camera Users with Disabilities} 
    &  
    High tolerance towards \newline camera-based assistive tech  & own experience of camera-based assistive tech; smartglasses as assistive tech; clear purpose; empathy; navigation; assistance; Aria \\ 
    \cline{2-3}
    &
    Tolerance to an extent  & no camera-based assistive tech at sensitive location; no 24/7 use; familiar place; no need to use; understand but not comfortable; confirm usage for assistive purpose; privacy policy of camera-based assistive tech \\ 
    \cline{2-3}
    &
    No additional tolerance  & no empathy; no difference from others; PVI can use camera for malicious purpose; judge based on one's own experience  \\ 
    \midrule
    %
     \multirow{8}{10em}{Complication in a Sighted World} 
    &  
    Privacy inequity between \newline BVI and sighted people & unfair; unequal information access as bystander; unequal info exchange; desire for equal access; PVI use camera with screen reader;   \\ 
    \cline{2-3}
    &
    Privacy not respected by \newline sighted people  & guide dog attract camera; become camera target; photo taken without notification \\ 
    \cline{2-3}
    &
    Weight others' privacy more  & sighed bystanders; other bystanders; sighted remote agent; worry about others' privacy \\
    \cline{2-3}
    &
    Hope for understanding \newline from sighted people  & importance of camera-based assistive tech; sighted people not understand; right to use camera as assistive tech; desire for understanding; proper communication for education; camera-based assistive tech as accepted norm \\ 
    \midrule
    %
    \multirow{8}{10em}{Expected Privacy Enhancements} 
    &  
    Info transparency and certainty & transparency of camera use; courtesy; information certainty; expected camera info; camera presence; camera range; camera purpose; whether oneself in camera; photo propagation; camera user; device type; camera location; modality of recorded info\\ 
    \cline{2-3}
    &
    Consent  & ask for consent \\ 
    \cline{2-3}
    &
    Desired privacy-enhancing tech  & necessity of privacy-enhancing tech; form factor; smartphone; smartwatch; necklace; wristband; audio feedback; haptic feedback; unobtrusive; proactive notification; pressure on users; low cost \\
    \cline{2-3}
    &
    Camera regulation policy \newline from sighted people  & workspace policy; policy by camera company; forced shutter sound\\ 
   
    \midrule
    \end{tabular}
%  }
    \caption{Themes and codebook in Study II.}
    \label{tab:codebook}
\end{figure*}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> 2-tables/tab_scenarios.tex <==
\begin{table*}[t]
\small
  \begin{tabular}{p{15cm} p{1.5cm}} 
    \toprule
    \textbf{Scenarios} 	& \textbf{Factors}\\
    \midrule
\textit{S1:} Your friends come to your house to visit you. Some of them use their smartphones to capture photos or videos. & \faIcon{mobile-alt} \hspace{0.1cm}  \faUserFriends  \hspace{0.1cm}  \faHouseUser	 \\
\midrule
\belowrulesepcolor{lightgray} 
\rowcolor{lightgray}\textbf{\textit{S2:} Someone from maintenance comes to your house to check the status of your air conditioner. They use their smartphone to capture photos or videos.}
  & \faIcon{mobile-alt} \hspace{0.1cm}  \faUserAstronaut \hspace{0.1cm}  \faHouseUser
\\
\aboverulesepcolor{lightgray}
\midrule
\textit{S3:} You are attending a meeting in your workplace. Some of your colleagues are using their smartphone to capture photos or videos.
& \faIcon{mobile-alt} \hspace{0.1cm}  \faUserFriends \hspace{0.1cm}  \faUmbrellaBeach
\\
\midrule
\textit{S4:} You are visiting a park, some strangers nearby are using their smartphones to capture photos or videos.
  & \faIcon{mobile-alt} \hspace{0.1cm}  \faUserAstronaut \hspace{0.1cm}  \faUmbrellaBeach
\\
\midrule
\belowrulesepcolor{lightgray} 
\rowcolor{lightgray}\textbf{\textit{S5:} You live with a roommate in an apartment. Your roommate always wears a pair of smartglasses with a camera in the apartment.}  & \faGlasses  \hspace{0.1cm}  \faUserFriends \hspace{0.1cm}  \faHouseUser
\\
\aboverulesepcolor{lightgray}
\midrule
\belowrulesepcolor{lightgray} 
\rowcolor{lightgray}\textbf{\textit{S6:} You walk in a public bathroom in a mall. A stranger in the bathroom wears a pair of smart glasses with a camera~\cite{CNet}. } & \faGlasses  \hspace{0.1cm}  \faUserAstronaut \hspace{0.1cm}  \faHouseUser
\\
\aboverulesepcolor{lightgray}
\midrule
\textit{S7:} You are attending the NFB convention. One of your friends nearby wears a pair of smart glasses with a camera.   & \faGlasses  \hspace{0.1cm}  \faUserFriends \hspace{0.1cm}  \faUmbrellaBeach
\\
\midrule
\textit{S8:} You are visiting a museum. A stranger nearby wears a pair of smart glasses with a camera~\cite{sprigg_2020}. & \faGlasses  \hspace{0.1cm}  \faUserAstronaut \hspace{0.1cm}  \faUmbrellaBeach
\\
\midrule
\textit{S9:} You walk into an elevator in your residency building. There is a security camera setup by the building admin.
 & \faVideo \hspace{0.1cm}  \faUserAstronaut \hspace{0.1cm}  \faHouseUser
\\
\midrule
\belowrulesepcolor{lightgray} 
\rowcolor{lightgray}\textbf{\textit{S10:} You are working in an open office. One of your colleagues who sits beside you set up a security camera on his or her desk.}  & \faVideo \hspace{0.1cm}  \faUserFriends \hspace{0.1cm}  \faUmbrellaBeach
\\
\aboverulesepcolor{lightgray}
\midrule
\textit{S11:} You are visiting a museum. There are security cameras setup by the museum in each exhibition section.  & \faVideo \hspace{0.1cm}  \faUserAstronaut \hspace{0.1cm}  \faUmbrellaBeach
\\
\midrule
\textit{S12:} You are living in an apartment in a residency building. You are familiar with your neighbor across the hallway. One day they installed a security camera at their front door.   & \faVideo \hspace{0.1cm}  \faUserFriends \hspace{0.1cm}  \faHouseUser
\\
\bottomrule
\end{tabular}
\caption{Twelve scenarios in Study I.} 
\label{tab:scenario}
\end{table*}


